A Probabilistic Graph Model for Trust Opinion Estimation in Online Social Networks

Trust assessment plays a key role in many online applications, such as online money lending, product reviewing and active friending. Trust models usually employ a group of parameters to represent the trust relation between a trustor-trustee pair. These parameters are originated from the trustor's bias and opinion on the trustee. Naturally, these parameters can be regarded as a vector. To address this problem, we propose a framework to accurately convert the single values to the parameters needed by 3VSL. The framework firstly employs a probabilistic graph model (PGM) to derive the trustor's opinion and bias to his rating on the trustee.

==> content/other.tex <==
\section{Introduction}  

Online Social Networks (OSNs) help people not only to strengthen their connections with known friends, but also to expand their social circle to friends of friends that they may not know previously.\\
%

One the other hand, the development of OSNs is also associated with the rise of OSNs spam attack. 
%
Therefore, OSNs spammer detection has attracted many attentions in recent years
%
Many previous efforts have been devoted to this problem~\cite{kim2012oto, yu2008sybilguard}. 
%
The basic principle of most previous work  is finding friend communities inside a social network and treating the nodes outside the community as suspicious users.  
%
However, recent studies~\cite{6547122} indicate that using topological information only to detect a friend community is not sufficient to identify spammers.
%
For example, many spammers pretend to be a normal user and broadcast friend requests in OSNs. 
%
They can be identified as a member of the community as long as few of their requests are accepted.\\   
%

In view of this limitation, we make use of trust in OSNs to identify spammers. 
%
The basic principle is that a friend's friend is trustworthy while an user whom my friends barely have interaction with is suspicious.
%
The assumption behind this idea is that normal users will never have strong social ties (messages, likes, ratings, etc.) with spammers, even though there is an edge between them.
%
In our previous work~\cite{6848107}, we proposed a trust model called 3VSL to assess the trustworthiness of a strange user in OSNs by propagating trust along the social ties among friends.      
%
3VSL defines trust as a \textit{probability} that a trustee will behave good as expected by a trustor. 
%
Such probability, which is called opinion, is expressed as a Dirichlet-Categorical distribution. 
%
Through aggregating and propagating opinions in OSNs, 3VSL is able to assess the trustworthiness of target users and identify spammers.  \\
%

A problem remaining to 3VSL is how to estimate the factors of an opinion. 
%
In other words, how to map social tie features such as messages, likes, ratings to the factors of Dirichlet-Categorical distribution, such that 3VSL model can give accurate result for spammer detection? Formally, we define the system model as followings:\\

\textit{A social interaction network is modeled as a feature matrix $V$ where an entry $V_{ij}$ is a feature vector $V_{ij}$. 
%
The feature vector $V_{ij}$ is composed of features collected from the interactions between user $i$ and $j$ on OSNs.
%
An opinion network is modeled as an opinion matrix $O$, where an entry $O_{ij}$ is an opinion from user $i$ to $j$.
%
The opinion is a tuple of factors expressing a certain Dirichlet-Categorical distribution.} \\
%

Then, the problem is formulated as:\\

%
\textit{Given a feature matrix $V$, how to estimate the opinion matrix $O$, upon which 3VSL model is able to conduct an accurate trust assessment for spammer detection.} 


==> new-commands.tex <==
\mathchardef\Gamma="0100 \mathchardef\Delta="0101
\mathchardef\Theta="0102 \mathchardef\Lambda="0103
\mathchardef\Xi="0104 \mathchardef\Pi="0105
\mathchardef\Sigma="0106 \mathchardef\Upsilon="0107
\mathchardef\Phi="0108 \mathchardef\Psi="0109
\mathchardef\Omega="010A

\newcommand{\ovspace}[1]{\vspace{#1}}

\newcommand{\outline}[1]{}%{\textbf{#1}}

\newcommand{\dl}{\mbox{$\, [ \hspace*{-1.5pt} [\,$}}
\newcommand{\dr}{\mbox{$\, ] \hspace*{-1.5pt} ]\:$}}
\newcommand{\da}{\mbox{$\, A \hspace*{-6.75pt} A \,$}}
%\newcommand{\drightarrow}{\mbox{$\rightarrow \hspace*{-8pt} \rightarrow$}}

\newcommand{\BA}{\mbox{${\bm{a}}$}}
%\newcommand{\BB}{\mbox{${\bm{c}}$}}
\newcommand{\BC}{\mbox{${\bm{c}}$}}
\newcommand{\BD}{\mbox{${\bm{d}}$}}
\newcommand{\BE}{\mbox{${\bm{e}}$}}
\newcommand{\BO}{\mbox{${\bm{o}}$}}
\newcommand{\BP}{\mbox{${\bm{p}}$}}
\newcommand{\BQ}{\mbox{${\bm{q}}$}}
\newcommand{\BR}{\mbox{${\bm{r}}$}}
\newcommand{\BV}{\mbox{${\bm{v}}$}}
\newcommand{\BL}{\mbox{${\bm{l}}$}}
\newcommand{\BI}{\mbox{${\bm{i}}$}}
\newcommand{\BH}{\mbox{${\bm{h}}$}}
\newcommand{\BS}{\mbox{${\bm{s}}$}}
\newcommand{\BB}{\mbox{${\bm{k}}$}}

\newcommand{\wrapbox}[1]{\framebox{\begin{tabular}{c}#1\end{tabular}}}
\newcommand{\CodeIn}[1]{{\small\texttt{#1}}}
\newcommand{\Section}[1]{Section~\ref{sec:#1}}
\newcommand{\SFigure}[2]{Figure~\ref{fig:#1}(#2)}

\usepackage{cite}
\usepackage{xspace}
\usepackage{url}
\usepackage{graphicx}
\usepackage{latexsym}
%\usepackage{amssymb}
%\usepackage{amsfonts}
%\usepackage{times}
\usepackage{psfrag}
\usepackage[tight]{subfigure}
\usepackage{wrapfig}
\usepackage{comment}
\usepackage[ruled,linesnumbered,vlined]{algorithm2e}
\usepackage{alltt}
\usepackage{color}
\usepackage{setspace}
\usepackage{rotating}
\usepackage{enumerate}
%\usepackage{algpseudocode}
%\usepackage{amsmath}

\newtheorem{defn}{Definition}[section]
\newtheorem{exmp}{Example}[section]
\newtheorem{thrm}{Theorem}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{lemm}{Lemma}[section]
\newtheorem{obsv}{Observation}[section]
\newtheorem{corr}{Corollary}[section]

%\addtolength{\textheight}{.23in} \addtolength{\textwidth}{.15in}
%\addtolength{\topmargin}{-.23in}
%\addtolength{\oddsidemargin}{.1in}
%\addtolength{\evensidemargin}{.1in}

\newtheorem{thm}{Theorem}
\newtheorem{dfn}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newcommand{\ie}{\emph{i.e.}\xspace}
\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\etc}{\emph{etc.}\xspace}
\newcommand{\etal}{\frenchspacing{}\emph{et al{.}}\xspace}
%\newcommand{\etal}[1]{{\sl et al.{#1}}}

%\newcommand{\thm}[1]{Theorem~\ref{thm:#1}}
%\newcommand{\lem}[1]{Lemma~\ref{lemma:#1}}
%\newcommand{cor}[1]{Corollary~\ref{cor:#1}}
\newcommand{\fac}[1]{Fact~\ref{fact:#1}}
\newcommand{\Table}[1]{Table~\ref{tab:#1}}
\newcommand{\Figure}[1]{Figure~\ref{fig:#1}}

%\theoremstyle{plain}
\newtheorem{property}{Property}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{theorem}{Theorem}[section]

%\theoremstyle{definition}
\newtheorem{notation}{Notation}
\newtheorem{Definition}{Definition}[section]

%\theoremstyle{remark}
\newtheorem{fact}{Fact}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{insight}{Insight}[section]

%%\algorithmstyle{definition}
%\algsetup{indent=1em}
%\renewcommand{\algorithmicrequire}{\textbf{Input:  }}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\factorial}{\ensuremath{\mbox{\sc Factorial}}}

\newcommand{\Comment}[1]{}

\renewcommand\floatpagefraction{0.999}
\renewcommand\topfraction{0.999}
\renewcommand\bottomfraction{0.999}
\renewcommand\textfraction{0.001}
\setcounter{totalnumber}{5}

